Learning-Based Near-Orthogonal Superposition Code for MIMO Short Message Transmission

Massive machine type communication (mMTC) has attracted new coding schemes optimized for reliable short message transmission. In this paper, a novel deep learning-based near-orthogonal superposition (NOS) coding scheme is proposed to transmit short messages in multiple-input multiple-output (MIMO) channels for mMTC applications. In the proposed MIMO-NOS scheme, a neural network-based encoder is optimized via end-to-end learning with a corresponding neural network-based detector/decoder in a superposition-based auto-encoder framework including a MIMO channel. The proposed MIMO-NOS encoder spreads the information bits to multiple near-orthogonal high dimensional vectors to be combined (superimposed) into a single vector and reshaped for the space-time transmission. For the receiver, we propose a novel looped K-best tree-search algorithm with cyclic redundancy check (CRC) assistance to enhance the error correcting ability in the block-fading MIMO channel. Simulation results show the proposed MIMO-NOS scheme outperforms maximum likelihood (ML) MIMO detection combined with a polar code with CRC-assisted list decoding by 1-2 dB in various MIMO systems for short (32-64 bit) message transmission.

==> discussion.tex <==
\section{Discussion}
%In this section, we will first discuss the desired codebook properties for the proposed looped $K$-best decoding to show the effectiveness of the MIMO-NOS, and further discuss the scalability of the proposed scheme.

%\subsection{Desired Codeword Property}
%??? Whether write it or not...

%\subsection{Scalability}
As shown in fig.\ref{fig:final_plot} (c), the polar baseline achieves nearly the same PER with the \textit{per-layer} sorting at $SNR=8dB$. We argue that the diminishing SNR gain is expected as polar code is capacity-achieving with large block length. On the other hand, for the MIMO-NOS scheme, the size of the neural encoders shown in fig.\ref{fig:network} grows linearly with the message length (with fixed $M$), which would result in performance degradation when optimizing the increasing number of parameters during training. Moreover, though proven to be capacity achieving when block length goes to infinity\cite{SPARC2014}, the simple superposition coding may be the bottleneck  fails to outperform other canonical channel codes (e.g., polar, LDPC and turbo codes) in medium block length. Nevertheless, the proposed MIMO-NOS is a promising solution for reliable short message transmission with MIMO in the low SNR regime with impressive PER performance and efficient decoding algorithm. Investigating a new DNN structure for the superposition code and its training scheme for longer information bit lengths is left as future work.
